Mixture-of-Thought-Tokens: Unifying Perception and Reasoning for Free-form Multimodal Grounding

Multimodal Large Language Models have made great progress in grounding tasks, yet existing methods still struggle to unify precise localization and complex reasoning. For one thing, text-based methods rely on coordinates or index prediction, severely limiting the perceptual capabilities of the model for dense visual objects. Meanwhile, latent token-based methods employ special tokens without inherent spatial references and use a decoding mechanism that lacks thinking steps, weakening high-level reasoning capabilities. Consequently, developing a unified framework that excels in both perception and reasoning remains challenging. To address this, we propose Mixture-of-Thought-Tokens (Motto), a new free-form multimodal grounding method that bridges the perception-reasoning gap, enabling MLLMs to empower diverse, arbitrary grounding queries. Specifically, we introduce Spatially-Grounded Thought Tokenization to explicitly align special tokens with spatial locations for clear spatial correspondence and visual interpretability. We further design a Context-Adaptive Chain-of-Tokens that dynamically switch grounding modes within an interleaved reasoning chain, achieving robust grounding across tasks of varying complexity. In addition, we construct PR-Bench, a new referring expression comprehension benchmark to evaluate the perception-reasoning gap. Extensive experiments demonstrate that Motto achieves state-of-the-art performance across diverse free-form grounding tasks.

==> tables/prbench.tex <==
% \begin{table}[]
% \centering
% \caption{The distribution of PR-Bench.}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{lccccccc}
% \toprule
% % \multicolumn{8}{c}{\textbf{PRBench}}                                                                                                                                                       
% \multirow{2}{*}{Type}& \multicolumn{3}{c}{Perception} & \multicolumn{3}{c}{Reasoning} & \multirow{2}{*}{Total}\\ 
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}
%     & Attribute & Position & Interaction & Relation & Commonsense & \multicolumn{1}{c}{Reject} &    \\ \midrule
% \multicolumn{1}{l}{Images}           & 701       & 735      & 642         & 695      & 715         & \multicolumn{1}{c}{764}    & 3102   \\
% \multicolumn{1}{l}{Phrases}       & 1,000     & 1,000   & 1,000  & 1,000   & 1,000 & \multicolumn{1}{c}{1,000}  & 6,000   \\
% \multicolumn{1}{l}{ Img Size}    & 1602x1301 & 1588x1294& 1608x1292   & 1619x1282& 1627x1280   & \multicolumn{1}{c}{1629x1301}& 1612x1292 \\
% \multicolumn{1}{l}{ Box Size}  & 10.76\%   & 8.34\%   & 9.43\%     & 6.15\%   & 6.14\%      & \multicolumn{1}{c}{N/A}    & 8.16\%  \\
% \multicolumn{1}{l}{Length}  & 9.3       & 11.0     & 10.3        & 14.4     & 15.5        & \multicolumn{1}{c}{13.8}     & 12.4    \\ 
% \bottomrule
% \end{tabular}%
% }
% \label{tab:prbench}
% \end{table}


% \begin{table}[]
% \centering
% \caption{The distribution of PR-Bench.}
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{llccccc}
% \toprule
% & Type & Images & Phrases & Image Size & Box Size & Phrase Length \\
% \midrule
% \multirow{3}{*}{Perception}
% & Attribute   & 701  & 1,000 & 1602$\times$1301 & 10.76\% & 9.3  \\
% & Position    & 735  & 1,000 & 1588$\times$1294 & 8.34\%  & 11.0 \\
% & Interaction & 642  & 1,000 & 1608$\times$1292 & 9.43\%  & 10.3 \\
% \midrule
% \multirow{3}{*}{Reasoning}
% & Relation    & 695  & 1,000 & 1619$\times$1282 & 6.15\%  & 14.4 \\
% & Commonsense & 715  & 1,000 & 1627$\times$1280 & 6.14\%  & 15.5 \\
% & Reject      & 764  & 1,000 & 1692$\times$1301 & N/A     & 13.8 \\
% \midrule
% & Total       & 3102 & 6,000 & 1612$\times$1292 & 8.16\%  & 12.4 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:prbench}
% \end{table}

\begin{table}[]
\centering
\caption{The distribution of PR-Bench.}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
 Type & Images & Phrases & Image Size & Box Size & Phrase Length \\
\midrule
\textbf{\textit{Perception}}\\
 Attribute   & 701  & 1,000 & 1602$\times$1301 & 10.76\% & 9.3  \\
 Position    & 735  & 1,000 & 1588$\times$1294 & 8.34\%  & 11.0 \\
 Interaction & 642  & 1,000 & 1608$\times$1292 & 9.43\%  & 10.3 \\
\midrule
\textbf{\textit{Reasoning}}\\
 Relation    & 695  & 1,000 & 1619$\times$1282 & 6.15\%  & 14.4 \\
 Commonsense & 715  & 1,000 & 1627$\times$1280 & 6.14\%  & 15.5 \\
 Reject      & 764  & 1,000 & 1692$\times$1301 & N/A     & 13.8 \\
\midrule
 Total       & 3102 & 6,000 & 1612$\times$1292 & 8.16\%  & 12.4 \\
\bottomrule
\end{tabular}
}
\label{tab:prbench}
\end{table}
